NoLiMa: Long-Context Evaluation Beyond Literal Matching

Recent large language models (LLMs) support long contexts ranging from 128K to 1M tokens. A popular method for evaluating these capabilities is the needle-in-a-haystack (NIAH) test, which involves retrieving a "needle" (relevant information) from a "haystack" (long irrelevant context). Extensions of this approach include increasing distractors, fact chaining, and in-context reasoning. However, in these benchmarks, models can exploit existing literal matches between the needle and haystack to simplify the task. To address this, we introduce NoLiMa, a benchmark extending NIAH with a carefully designed needle set, where questions and needles have minimal lexical overlap, requiring models to infer latent associations to locate the needle within the haystack. We evaluate 13 popular LLMs that claim to support contexts of at least 128K tokens. While they perform well in short contexts (<1K), performance degrades significantly as context length increases. At 32K, for instance, 11 models drop below 50% of their strong short-length baselines. Even GPT-4o, one of the top-performing exceptions, experiences a reduction from an almost-perfect baseline of 99.3% to 69.7%. Our analysis suggests these declines stem from the increased difficulty the attention mechanism faces in longer contexts when literal matches are absent, making it harder to retrieve relevant information. Even models enhanced with reasoning capabilities or CoT prompting struggle to maintain performance in long contexts. We publicly release the dataset and evaluation code at https://github.com/adobe-research/NoLiMa.

==> Figures/normal_vs_inverted.tex <==
\begin{figure}[t!]
    \centering
    \subfigure{
    % trim: left bottom right top
        \includegraphics[width=0.48\linewidth, trim=10 8 10 8, clip] {Figures/files/normal_vs_inverted_small.pdf}
    }
    \caption{Normalized performance comparison of normal and inverted examples across the GPT-4o and Llama 3.3 70B models. The red dotted line indicates the 0.85 effective threshold.}
    \label{fig:normal_vs_inverted}
\end{figure}

==> Figures/twoHop_vs_oneHop.tex <==
\begin{figure}[h!]
    \centering
    \subfigure{
        \includegraphics[width=0.88\linewidth, trim=10 10 10 8, clip] {Figures/files/onehop_vs_twohop.pdf}
    }
    \caption{Comparison of one-hop vs. two-hop normalized performance across GPT-4o and Llama 3.3 70B models. The red dotted line indicates the 0.85 effective threshold.}
    \label{fig:one_vs_twohop}
\end{figure}

==> Tables/model_results_w_64K_and_128K.tex <==
\begin{table*}[h!]
        \small
	\setlength\tabcolsep{5pt}
	\centering
	\begin{tabular}{l|cc|ccccccccc}
		\toprule
        \multirow{2}{*}{\textbf{Models}} & \textbf{Claimed} & \textbf{Effective} & \textbf{Base Score} & \multirow{2}{*}{\textbf{1K}} & \multirow{2}{*}{\textbf{2K}} & \multirow{2}{*}{\textbf{4K}} & \multirow{2}{*}{\textbf{8K}} & \multirow{2}{*}{\textbf{16K}} & \multirow{2}{*}{\textbf{32K}} & \multirow{2}{*}{\textbf{64K}} & \multirow{2}{*}{\textbf{128K}\footnotemark} \\
        & \textbf{Length} & \textbf{Length} & ($\times$0.85: \textbf{Thr.}) &&&&&&&& \\
        \midrule
        GPT-4o              & 128K & 8K & 99.3 (84.4) & \underline{98.1} & \underline{98.0} & \underline{95.7} & \underline{89.2} & 81.6 & 69.7 & 62.4 & 56.0 \\
        Gemini 2.0 Flash   & 1M   & 4K & 89.4 (76.0) & \underline{87.7} & \underline{87.5} & \underline{77.9} & 64.7 & 48.2 & \cellcolor[HTML]{faa7a7}41.0 & \cellcolor[HTML]{faa7a7}33.0 & \cellcolor[HTML]{faa7a7}16.4 \\
		\bottomrule
	\end{tabular}
	\caption{\framework benchmark results for GPT-4o and Gemini 2.0 Flash, covering extended context lengths of 64K and 128K. Scores above the effective threshold are underlined, while scores that are below 50\% of the base score are shaded in \colorbox{shadedRed}{red}.}
	\label{tab:models_performance_w_64K_and_128K}
\end{table*}


